Asymptotic Analysis of Deep Residual Networks

We investigate the asymptotic properties of deep Residual networks (ResNets) as the number of layers increases. We first show the existence of scaling regimes for trained weights markedly different from those implicitly assumed in the neural ODE literature. We study the convergence of the hidden state dynamics in these scaling regimes, showing that one may obtain an ODE, a stochastic differential equation (SDE) or neither of these. In particular, our findings point to the existence of a diffusive regime in which the deep network limit is described by a class of stochastic differential equations (SDEs). Finally, we derive the corresponding scaling limits for the backpropagation dynamics.

==> sec/7_conclusion.tex <==
 \section{Conclusion}
 
 We have provided empirical and theoretical evidence for the existence of at least three different scaling regimes for Residual Networks with many layers as the number of layers increases. We also theoretically characterize the ODE and SDE limits for the hidden state dynamics in deep fully-connected residual networks.

 In the first regime, rescaled network weights depend continuously on the layer. We show that in this case, the hidden state dynamics are asymptotically described by an ordinary differential equation, albeit one different from the neural ODE behavior. A second regime corresponds to the case where the rescaled weights may be decomposed into a continuous function of the layer plus a noise term. The dynamics of the hidden state are then asymptotically described either by a stochastic differential equation or an ordinary differential equation with random coefficients. A third case is the {\it sparse} regime, observed for convolutional architectures, in which a finite number of weights retain large amplitudes while others are close to zero.
 
% {\color{red}[??] These findings have interesting implications for the training of such large-scale networks in the first two regimes: we have shown that... xXX}
 
%Our work contributes to a better understanding of the behavior of residual networks and the role of the depth. Our findings point to interesting questions regarding the asymptotic behavior of such networks in the case of non-smooth activation functions and more complex architectures.


{ We also characterize the asymptotic behaviour of the backpropagation dynamics in terms of  backward ODE and SDE limits. In the diffusive regime, we derive the limiting equation at optimality. 

Our results contribute to a better understanding of the behavior of residual networks in the deep network limit, with an emphasis on the role of network depth in such architectures, and points to various open questions regarding the asymptotic behavior of such networks in the case of non-smooth activation functions and more complex architectures, which remain to be explored. }

==> sec/OLD_wrong_proof_of_thm5.tex <==
\subsubsection{Old and wrong proof of Theorem~\ref{thm:backward-H2}}\label{sec:proof_backward-H2}

\begin{thm}[Backpropagation limit under Hypothesis~\ref{hypothesis.2} for \textbf{optimal weights}]\label{thm:backward-H2}Let Assumptions~\ref{ass:activation}, \ref{ass:ito}, \ref{ass:strong}, and~\ref{ass:backward} hold true and let $\alpha=0$ and $\beta = 1$. We assume that there exists $C, \zeta > 0$ such that for each $L$ big enough, the weights $\theta^{(L)}$ satisfy the optimality condition:
\begin{equation} \label{eq:optimality-condition}
\E \left[ \sup_{x\in B} \norm{ \nabla_x \hspace{-1pt} \left( \phi_{\theta^{(L)}} - \ftrue \right)(x) }^4 \right] < C L^{-4-\zeta}.
\end{equation}
Suppose that there exists a solution $(H_t)_{t\in\left[0,1\right]}$ to the SDE \eqref{eq:limit1}, and a process $(G_t)_{t\in\left[0,1\right]}$ satisfying $\E\left[ \sup_{t\in\left[0,1\right]} \norm{G_t}^p \right] < \infty$ that solves the SDE: $G_0 = \nabla_x \ftrue(x)$, $G_1 = I_d$, and
\begin{eqnarray}\label{eq:backward-3}
-\dd G_t = \left( \overbar{A}_t G_t + \frac{1}{2} \sigma''(0) \frac{\del Q}{\del x}(t, H_t) G_t \right) \dd t + \dd\hspace{-2pt} \left[W^A, G\right]_t + \dd W^A_t G_t.
\end{eqnarray}
Then, backpropagation dynamics $\overbar{G}^{(L)} = \sum_{k=0}^{L-1} g_k^{(L)} \one_{\left[ t_k, t_{k+1}\right)}$ converge uniformly in $L^2$ to $G$.
\end{thm}


The ideas of the proof follow closely those of Theorem~\ref{thm:H2}, and we will provide here the main arguments. For the ease of notation exposition, we consider $U=0$ and we use $C$ to denote some generic constant (independent from $L$ and other parameters, such as $\varepsilon$, $\delta$, and $R$, to be defined later) that may vary from step to step. 

{\color{blue} The proof consists of 15 steps that can be summarized as follows. Step 1 is concerned with rewriting the backpropagation equation to distinguish the drift terms, the stochastic terms, and the error terms. Step 2 defines the \textit{continuous-time approximation} (CTA) of $G$, and step 3 proves that the CTA is uniformly close to $g^{(L)}_k$. Step 4 and 5 provide early calculations to show a uniform bound between the CTA and $G$. Step 6 and 7 use the optimality condition to handle the Ito integral and the quadratic covariation terms. Step 8 proves that one of the error terms, the Taylor remainder, uniformly vanishes. Step 9 decomposes the Ito remainder term into five different quantities. Step 10, 11 and 12 prove that these 5 quantities uniformly vanish. Step 13 proves that a stochastic cross-term also vanishes uniformly. Step 14 deals with the drift error between choosing the left and the right point for the integral. Step 15 wraps up everything and finishes the proof. \\
}

\noindent \underline{Step 1: Rewrite the discrete backpropagation equation.} First, for each $i, j=1, \ldots, d$, \eqref{eq:backprop} gives \[ 
 g_{k, ij}^{(L)} = g_{k+1, ij}^{(L)} + \sum_{l=1}^d \sigma' \hspace{-2pt} \left( A_k^{(L)} h_{k}^{(L)} + b_k^{(L)} \right)_i A^{(L)}_{k, il}  g_{k+1, lj}^{(L)}.
\]
By Taylor's theorem on $\sigma'$, {as $\sigma'''$ is continuous}, there exists $\xi_{k, i}^{(L)} \in \left[0, \left(A_k^{(L)} h_{k}^{(L)} + b_k^{(L)}\right)_i \right]$ such that
\begin{align*}
    \sigma'\left( A_k^{(L)} h_{k}^{(L)} + b_k^{(L)} \right)_i &= \sigma'(0) + \sigma''(0) \left( A_k^{(L)} h_{k}^{(L)} + b_k^{(L)} \right)_i + \frac{1}{2} \sigma''' \hspace{-2pt} \left( \xi_{k, i}^{(L)} \right) \left( A_k^{(L)} h_{k}^{(L)} + b_k^{(L)} \right)_i^2.
\end{align*}
Hence, using $\sigma'(0)=1$, we get 
\begin{align*}
    g_{k,ij}^{(L)} &= g_{k+1, ij}^{(L)} + \left( A^{(L)}_k g_{k+1}^{(L)} \right)_{ij} + \sigma''(0) \sum_{m,l=1}^d A^{(L)}_{k, im} A^{(L)}_{k, il} h^{(L)}_{k, m} g^{(L)}_{k+1, lj} + \sigma''(0) b^{(L)}_{k,i} \left( A^{(L)}_k g_{k+1}^{(L)} \right)_{ij} \\
    &+ \frac{1}{2} \sigma'''\hspace{-2pt} \left( \xi_{k, i}^{(L)} \right) \left( A_k^{(L)} h_{k}^{(L)} + b_k^{(L)} \right)_i^2 \left( A^{(L)}_{k} g_{k+1}^{(L)} \right)_{ij} \\
    &= g_{k+1, ij}^{(L)} + \left[ \left( \overbar{A}_{t_k} + \frac{1}{2} \sigma''(0) \frac{\del Q}{\del x}\left(t_k, H_{t_k}\right) \right) g_k^{(L)} \right]_{ij} L^{-1} + \left( \Delta W^A_k  g_{k+1}^{(L)} \right)_{ij} + D_k^{(L)}\hspace{-2pt} \left( g_{k+1}^{(L)} \right)_{ij} \\
    &= g_{k+1, ij}^{(L)} + \nu\hspace{-1pt}\left(t_k, g_k^{(L)} \right)_{ij} L^{-1} + \left( \Delta W^A_k  g_{k}^{(L)} \right)_{ij} + \left( \Delta W^A_k  \Delta \overbar{G}_{k}^{(L)} \right)_{ij} + D_k^{(L)}\hspace{-2pt} \left( g_{k+1}^{(L)} \right)_{ij}
\end{align*}
where \begin{equation} \label{def:mu-thm5}
\nu(t, g) \coloneqq \overbar{A}_t g + \frac{1}{2} \sigma''(0) \frac{\del Q}{\del x}(t, H_t) g %+ \sigma''(0) \Sigma_t^{A, b}(g).
\end{equation}
and 
\begin{equation}
\begin{aligned}\label{eq:D_R_N}
D_k^{(L)}\hspace{-2pt}\left( g \right) &\coloneqq N^{(L),1}_{k}\hspace{-2pt}\left( g \right) + N^{(L),2}_{k}\hspace{-2pt} \left( g \right) + N^{(L),3}_{k}(g) + R_k^{(L)}\hspace{-2pt}\left( g \right), \\
N^{(L), 1}_{k, ij}\hspace{-2pt} \left( g \right) &\coloneqq \sigma''(0) \left( \sum_{m,l=1}^d A^{(L)}_{k, im} A^{(L)}_{k, il} h^{(L)}_{k, m} g_{lj} - \frac{1}{2} \left( \frac{\del Q}{\del x}\left(t_k, H_{t_k}\right) g \right)_{ij} L^{-1} \right), \\
N^{(L), 2}_{k, ij}\hspace{-2pt} \left( g \right) &\coloneqq \sigma''(0) b^{(L)}_{k,i} \left( A^{(L)}_k g \right)_{ij} \\
N^{(L),3}_{k}(g) &\coloneqq \nu\hspace{-1pt}\left(t_k, g - g_k^{(L)} \right) L^{-1} \\
R_{k, ij}^{(L)}(g) &\coloneqq \frac{1}{2} \sigma'''\hspace{-2pt} \left( \xi_{k, i}^{(L)} \right) \left( A_k^{(L)} h_{k}^{(L)} + b_k^{(L)} \right)_i^2 \left( A^{(L)}_{k} g \right)_{ij}. 
\end{aligned}    
\end{equation}
We write the recurrence equation above in terms of $g_{k}^{(L)}$ instead of $g_{k+1}^{(L)}$ as our target limit $G$ is adapted to the forward filtration generated by the Ito processes $W^A$ and $W^b$. \\


\noindent \underline{Step 2: Continuous-time approximation.} Now, we rewrite the target SDE limit as \[
    - \dd G_t = \nu(t, G_t) \dd t + \dd \hspace{-2pt} \left[W^A, G\right]_t + \dd W_t^A G_t.
\]
Let $k_s$ the index for which $t_{k_s} \leq s < t_{k_s+1}$. Define the \textit{continuous-time approximation} \[
    \widetilde{G}_t^{(L)} \coloneqq I_d - \int_t^T \nu \hspace{-1pt} \left( t_{k_s}, \overbar{G}^{(L)}_s \right) \dd s - \int_t^T \dd W_s^A \overbar{G}^{(L)}_s - \sum_{k > Lt-1} \left( \Delta W^A_k  \Delta \overbar{G}_{k}^{(L)} + D_k^{(L)}\hspace{-2pt} \left( g_{k+1}^{(L)} \right) \right).
\]
By definition, we directly have $\widetilde{G}_{t_k}^{(L)} = \overbar{G}_{t_k}^{(L)} = g_k^{(L)}$. Note that the Ito integral term is in fact a finite sum, so is well-defined even though $\overbar{G}^{(L)}_s$ is not a priori adapted.

{$\widetilde{G}_{t_k}^{(L)}$ is used as an intermediate quantity to prove the theorem. To show that the difference between $G$ and $\overbar{G}$ is uniformly bounded, we first show that $\overbar{G}^{(L)} - \widetilde{G}^{(L)}$ is uniformly bounded (in Step 3) and then show that $G - \widetilde{G}^{(L)}$ is uniformly bounded (in Steps 4-14).}\\

\noindent \underline{Step 3: Uniform bound between $\overbar{G}^{(L)}$ and $\widetilde{G}^{(L)}$.} We have, for $s\in\left[ 0, 1 \right]$, 
\begin{align*}
\norm{ \widetilde{G}^{(L)}_s - \overbar{G}^{(L)}_s }^2 &= \norm{ \nu\hspace{-1pt} \left(t_{k_s}, g_{k_s}^{(L)}\right) (s - t_{k_s}) + \left( W^A_{s} - W^A_{t_{k_s}} \right) g_{k_s}^{(L)} }^2 \\
&\leq 2C \left(1+\sup_{t\in\left[0,1\right]} \norm{H_t}^2 \right) \norm{g_{k_s}^{(L)}}^2 L^{-2} + 2 \norm{ \left( W^A_{s} - W^A_{t_{k_s}} \right) g_{k_s}^{(L)} }^2.
\end{align*}
Hence, 
\begin{align*}
    \E\left[ \sup_{0\leq s \leq 1} \norm{ \widetilde{G}^{(L)}_s - \overbar{G}^{(L)}_s }^2  \right] &\leq 2C \,\, \E\left[ \left(1+\sup_{t\in\left[0,1\right]} \norm{H_t}^2 \right)^2 \right]^{1/2} \E\left[ \sup_k \norm{g_k^{(L)}}^4 \right]^{1/2} L^{-2} \\
    &\quad+ 2 \, \E\left[ \sup_k \norm{g_k^{(L)}}^4 \right]^{1/2} \E\left[ \sup_{0\leq s \leq 1} \norm{ W^A_{s} - W^A_{t_{k_s}} }^4 \right]^{1/2}.
\end{align*}
By Assumptions~\ref{ass:strong} and \ref{ass:backward}, and equation~\eqref{eq:bound16}:
\begin{equation} \label{eq:unif-bound-bar-tilde}
\E\left[ \sup_{0\leq s \leq 1} \norm{ \widetilde{G}^{(L)}_s - \overbar{G}^{(L)}_s }^2  \right] < C L^{-1}.
\end{equation}

\noindent \underline{Step 4: Definition of useful high-probability events.} Recall the following discrete filtration \[
\GG_{k} \coloneqq \sigma\Big(q_s^A,q_s^b, B_s^{A}, B_s^{b} \,:\,\, s \leq t_{k+1} \Big).
\]
In order to prove a uniform bound between $G$ and $\widetilde{G}^{(L)}$, we define events under which the computations simplify. Let $R > 1$. For $k=0, \ldots, L$, define
\begin{equation}  \label{eq:events-E} 
    \widetilde{E}_{k, R}^{(L)} \coloneqq \left\{ \sup_{t\in\left[t_{k-1}, t_{k}\right]} \norm{H_t} \leq R \right\} \cap \left\{ \norm{h_{k}^{(L)}} \leq R \right\}, \,\, E_{k, R}^{(L)} \coloneqq \bigcap_{k'=0}^k \widetilde{E}_{k', R}^{(L)}, \,\, E_R^{(L)} \coloneqq E_{L, R}^{(L)}.
\end{equation}
From \eqref{eq:bound5}, we know that $\Prob\left( (E_R^{(L)})^c \right) \leq C R^{-p}$. Further, define for $k=0, \ldots, L-1$ the following events:
\begin{equation} \label{eq:events-F}
    \widetilde{F}^{(L)}_{k, R} \coloneqq \left\{ \norm{A_{k}^{(L)}} \leq 1/R \right\} \cap \left\{ \norm{b_{k}^{(L)}} \leq 1 \right\}, \quad F^{(L)}_{k, R} \coloneqq \bigcap_{k'=0}^k \widetilde{F}^{(L)}_{k', R}, \quad F^{(L)}_R \coloneqq F^{(L)}_{L-1,R}. 
\end{equation}
We prove that under $E^{(L)}_{k,R} \cap F^{(L)}_{k,R} \in \GG_{k}$, the Jacobian matrices linking $g_k^{(L)}$ and $g_{k+1}^{(L)}$ in \eqref{eq:backprop} are invertible. 

\begin{lem} \label{lemma:invertible-events}
Let $D_k^{(L)} \coloneqq \diag\left( \sigma'_d \hspace{-1pt} \left( A_{k}^{(L)} h_{k}^{(L)} + b_{k}^{(L)} \right) \right) A^{(L)}_{k} \in \R^{d\times d}$. Then, for $R > 2C_1$ with $C_1 \coloneqq \left( 1 + 2\abs{\sigma''(0)} + 2 \sup \abs{\sigma'''} \right)$, we have:
\begin{enumerate}[label=(\roman*)]
    \item $\widetilde{E}^{(L)}_{k,R} \cap \widetilde{F}^{(L)}_{k,R} \subseteq \left\{ I_d + D_{k}^{(L)} \, \text{is invertible} \right\}$.
    \item There exists $C>0$ such that $\Prob\left( F^{(L)}_R \right) > 1 - L \exp\left( -C(LR^{-1} - 1)^2\right) $.
\item {$\norm{\left(I_d +  D_{k}^{(L)}\right)^{-1}} \one_{\widetilde{E}^{(L)}_{k,R} \cap \widetilde{F}^{(L)}_{k,R}} \leq 1+\frac{C_1}{R-C_1}$.}
\end{enumerate}
\end{lem}
\begin{proof}
For $(i)$, we use the fact that if a matrix $D\in\R^{d\times d}$ satisfies $\norm{D}_2 < 1$, then $I_d + D$ is invertible. Observe that 
\begin{align*}
    \norm{D_k^{(L)}}_2 \coloneqq \norm{ \diag\left( \sigma'_d \hspace{-1pt} \left( A_{k}^{(L)} h_{k}^{(L)} + b_{k}^{(L)} \right) \right) A^{(L)}_{k} }_2 \leq \max_i \abs{ \sigma'\hspace{-1pt}\left( A_{k}^{(L)} h_{k}^{(L)} + b_{k}^{(L)} \right)_i } \norm{A_{k}^{(L)}}_2.
\end{align*}
By Taylor's theorem, there exists $\xi^{(L)}_{k, i} \in \R$ such that 
\begin{equation*}
    \sigma'\hspace{-1pt}\left( A_k^{(L)} h_k^{(L)} + b_k^{(L)} \right)_i = 1 + \sigma''(0) \left( A_k^{(L)} h_k^{(L)} + b_k^{(L)} \right)_i + \frac{1}{2} \sigma'''\hspace{-2pt}\left( \xi^{(L)}_{k, i} \right) \left( A_k^{(L)} h_k^{(L)} + b_k^{(L)} \right)_i^2.  
\end{equation*}
Hence, under $\widetilde{E}^{(L)}_{k,R} \cap \widetilde{F}^{(L)}_{k,R}$, we have 
\begin{equation}
    \norm{D_k^{(L)}}_2 \leq \left( 1 + 2\abs{\sigma''(0)} + 2 \sup \abs{\sigma'''} \right) R^{-1} \eqqcolon C_1 R^{-1}.  \label{eq:Dbound}
\end{equation}
So $\norm{D_{k}^{(L)}}_2 \one_{\widetilde{E}^{(L)}_{k,R} \cap \widetilde{F}^{(L)}_{k,R}} < 1$ for each $k=0, \ldots, L-1$. \\ 

\noindent For $(ii)$, the union bound gives directly
\begin{align*}
    \Prob\left((F^{(L)}_R)^{c} \right) \leq \sum_{k=0}^{L-1} \Prob\left( \norm{A_{k}^{(L)}} > 1/R  \right) + \Prob\left( \norm{b_{k}^{(L)}} > 1  \right).  
\end{align*}
Next, we use Chernoff bounds on the tails of a Gaussian distribution:
\begin{align*}
\Prob\left( \norm{A_{k}^{(L)}} > 1/R  \right) &\leq \Prob\left( \norm{\Delta W^A_{k} } > R^{-1} - CL^{-1} \right) \leq \exp\left( -C(LR^{-1} - 1)^2\right), \\
\Prob\left( \norm{b_{k}^{(L)}} > 1  \right)   &\leq \Prob\left( \norm{\Delta W^b_{k} } > 1 - CL^{-1} \right) \leq \exp\left( -C(L - 1)^2\right).
\end{align*}
Hence, as $R > 1$, $\Prob\left((F^{(L)}_{R})^{c} \right) \leq L \exp\left( -C(LR^{-1} - 1)^2\right)$.

\noindent For (iii), assume that event $\widetilde{E}^{(L)}_{k,R} \cap \widetilde{F}^{(L)}_{k,R}$ holds. By rearranging the terms, we have \[
D_k^{(L)}\left( D_k^{(L)}+I_d \right)^{-1} = \left( D_k^{(L)}+I_d-I_d\right) \left( D_k^{(L)}+I_d \right)^{-1} = I_d - \left( D_k^{(L)}+I_d \right)^{-1}.
\]
Hence $\left( D_k^{(L)}+I_d \right)^{-1} = I_d - D_k^{(L)} \left( D_k^{(L)}+I_d \right)^{-1}$. Therefore
\begin{eqnarray*}
\norm{\left(D_k^{(L)}+I_d\right)^{-1}} \leq \norm{I_d} + \norm{D_k^{(L)} \left( D_k^{(L)}+I_d \right)^{-1}} \leq \norm{I_d} + \norm{D_k^{(L)}} \norm{ \left( D_k^{(L)}+I_d \right)^{-1}}.
\end{eqnarray*}
We have $\norm{D_k^{(L)}}\leq C_1 R^{-1}$ from \eqref{eq:Dbound}. We have as well, as $R \ge 2C_1$,
\begin{eqnarray*}
\norm{\left(D_k^{(L)}+I_d\right)^{-1}} \leq \frac{ \norm{I_d} }{1-\norm{D_k^{(L)}}} \leq \frac{R}{R-C_1} = 1+\frac{C_1}{R-C_1}.
\end{eqnarray*}
\end{proof}
\noindent As a corollary, under $E^{(L)}_{k-1,R} \cap F^{(L)}_{k-1,R}$, we are allowed to write 
\begin{equation} \label{eq:rewrite-gradients}
    g^{(L)}_k = \left( \prod_{k'=0}^{k-1} \left( I_d + D_{k'}^{(L)} \right)^{-1} \right) g^{(L)}_0 \eqqcolon J_k^{(L)} g^{(L)}_0.  
\end{equation}
Hence, as $D_k^{(L)}$ is $\GG_{k}-$measurable, we deduce that $J_k^{(L)}$ is $\GG_{k-1}-$measurable. \\

\noindent \underline{Step 5: Initial computations for a uniform bound between $G$ and $\widetilde{G}^{(L)}$.} Fix $\epsilon > 0$, and let $\delta > 0$ (to be determined later) that only depends on $L$ and $\epsilon$. Using Assumption~\ref{ass:backward}, we have similarly to \eqref{eq:bound1} that 
\begin{align} 
    \mathbb{E}\left[ \sup_{0 \leq t \leq 1} \norm{G_t - \widetilde{G}^{(L)}_t}^2 \right] & \leq \mathbb{E}\left[ \sup_{0 \leq t \leq 1} \norm{G_t - \widetilde{G}^{(L)}_t}^2 \one_{E^{(L)}_R \cap F^{(L)}_R} \right] \nonumber \\
    &+\frac{2^{p+1}\delta C}{p} + \frac{1-2/p}{\delta^{2/(p-2)}} \left( \Prob\left( ( E_R^{(L)})^c \right) + \Prob\left( ( F_R^{(L)})^c \right) \right). \label{eq:bound-eg}
\end{align}
Next, we first estimate, for $t\in\left[0,1\right]$,
\begin{align}
    \norm{G_t - \widetilde{G}^{(L)}_t}^2 &\leq 4 \int_t^T \norm{\nu(t_{k_s}, \overbar{G}_s^{(L)}) - \nu(s, G_s)}^2 \dd s + 4 \norm{ \int_t^T  \dd W^A_s \left(\overbar{G}_s^{(L)} - G_s \right) }^2 \nonumber \\
    &+ 4 \norm{ \left[W^A, G\right]_{\cdot} \Big\vert^{T}_{t} - \sum_{k>Lt-1} \Delta W^A_k  \Delta \overbar{G}_{k}^{(L)} }^2 +  4 \norm{ \sum_{k > Lt-1} D_k^{(L)} \hspace{-2pt} \left( g_{k+1}^{(L)} \right) }^2. \label{eq:unif-bound-tilde-1}
\end{align}
The goal is to bound the first three terms as a function of the $L^2$ distance between $G$ and $\overbar{G}$ and terms vanishing uniformly in $L$, and show that the fourth term uniformly vanishes in $L$. To handle the term involving the drift $\nu$, we first prove the following lemma. 
\begin{lem} \label{lem:drift-lipschitz}
There exists $C>0$ such that for $t_1, t_2 \in \left[0, T\right]$ and $g_1, g_2 \in \R^{d \times d}$, 
\begin{align*}
    \norm{ \nu(t_2, g_2) - \nu(t_1, g_1) }^2 &\leq C \Big(1 + \sup_{t\in\left[0,1\right]} \norm{H_t}^2 \Big) \left(  \norm{g_2 - g_1}^2 + \norm{g_1}^2 \abs{t_2 - t_1}^{\kappa} \right)
\end{align*}
\end{lem}
\begin{proof}
It is a direct estimation: $\nu$ is linear in $g$ and a.s. H\"older with constant $\kappa$ in $t$.
\begin{align*}
    \norm{ \nu(t_2, g_2) - \nu(t_1, g_1) }^2 &\leq 2\norm{\nu(t_2, g_2) - \nu(t_2, g_1)}^2 + 2 \norm{\nu(t_2, g_1) - \nu(t_1, g_1)}^2 \\
    &\leq C \Big(1 + \sup_{t\in\left[0,1\right]} \norm{H_t}^2 \Big)  \norm{g_2 - g_1}^2 \\
    &+ 4 \norm{g_1}^2 \left( \norm{\overbar{A}_{t_2} - \overbar{A}_{t_1}}^2 + \frac{1}{2}\sigma''(0)\norm{\frac{\del Q}{\del x}(t_2, H_{t_2}) - \frac{\del Q}{\del x}(t_1, H_{t_1})}^2 \right)
\end{align*}
Now, $\frac{\del Q}{\del x}$ is linear in $x$, and $H_t$ has a.s $\gamma-$H\"older-continuous paths, for all $\gamma<\kappa+1/2$. Hence, \[
    \norm{\frac{\del Q}{\del x}(t_2, H_{t_2}) - \frac{\del Q}{\del x}(t_1, H_{t_1})}^2 \leq C \Big(1 + \sup_{t\in\left[0,1\right]} \norm{H_t}^2 \Big)  \abs{t_2 - t_1}^{\kappa}. 
\]
\end{proof}
\noindent We directly deduce that 
\begin{align}
\E\left[ \one_{E^{(L)}_R} \int_0^T \norm{\nu(t_{k_s}, \overbar{G}_s^{(L)}) - \nu(s, G_s)}^2 \dd s \right] &\leq C(1+R^2) \, \E\left[ \int_0^T \norm{\overbar{G}_s^{(L)} - G_s}^2 \dd s \right] \nonumber \\
&+ C (1+R^2) \, \E\left[ \int_0^T \norm{\overbar{G}_s^{(L)}}^2 \abs{ t_{k_s} - s}^{\kappa} \dd s \right]. \label{eq:bound-mu}
\end{align}

\noindent For the second term in \eqref{eq:bound-mu} we immediately get
\begin{equation*}
\E\left[ \int_0^T \norm{\overbar{G}_s^{(L)}}^2 \abs{ t_{k_s} - s}^{\kappa} \dd s \right] \leq \E\left[ \sup_k \norm{g_k^{(L)}}^2 \right] \int_0^T \abs{ t_{k_s} - s}^{\kappa} \dd s \leq C L^{-\kappa}. 
\end{equation*}
Hence, we obtain from \eqref{eq:unif-bound-tilde-1} 
\begin{align}
&\E\left[ \sup_{0\leq t \leq 1} \norm{G_t - \widetilde{G}^{(L)}_t}^2  \one_{E^{(L)}_R \cap F^{(L)}_R}  \right] \nonumber \\
&\leq C(1+R^2) L^{-\kappa} +  4 \, \E\left[ \sup_{0\leq t \leq 1} \norm{ \int_t^T \dd W^A_s \left( \overbar{G}_s^{(L)} - G_s \right)  }^2 \one_{E^{(L)}_R \cap F^{(L)}_R} \right] \nonumber \\
&+ 4 \E \left[ \sup_{0\leq t < 1} \norm{ \left[W^A, G\right]_{\cdot} \Big\vert^{T}_{t} - \sum_{k>Lt-1} \Delta W^A_k  \Delta \overbar{G}_{k}^{(L)} }^2 \one_{E^{(L)}_R \cap F^{(L)}_R} \right] \nonumber \\
&+ 4 \, \E\left[ \sup_{0\leq t\leq 1} \norm{ \sum_{k > Lt-1} D_k^{(L)} \hspace{-2pt} \left( g_{k+1}^{(L)} \right) }^2  \one_{E^{(L)}_R \cap F^{(L)}_R} \right] \label{eq:unif-bound-tilde-2}
\end{align}
For the second term, we want to use Doob's martingale inequality, but $\overbar{G}_s^{(L)}$ is not adapted. We use the optimality assumption to deal with it in Step 6. For the third term, we construct an appropriate martingale in Step 7 and use the optimality assumption in the same fashion. To bound the fourth term in \eqref{eq:unif-bound-tilde-2}, recall that $D_k^{(L)}$ is decomposed into four terms $R^{(L)}_k$, $N^{(L),1}_k$, $N^{(L),2}_k$ and $N^{(L),3}_k$ in \eqref{eq:D_R_N}. We first bound the Taylor remainder $R^{(L)}_k$ in Step 8, the stochastic reminder terms $N^{(L),1}_k$ and $N^{(L),2}_k$ in Steps 9-13, and finally the drift error term $N^{(L),3}_k$ in Step 14.  \\

\noindent \underline{Step 6: Use the optimality condition \eqref{eq:optimality-condition} to handle the Ito integral term.} Recall from \eqref{eq:unif-bound-tilde-2} that we need to estimate
\begin{equation} \label{eq:ito-integral-cond-EF}
    \E\left[ \sup_{0\leq t \leq 1} \norm{ \int_t^T \dd W^A_s \left( \overbar{G}_s^{(L)} - G_s \right)  }^2 \one_{E^{(L)}_R \cap F^{(L)}_R} \right].
\end{equation}
Conditioning on the event $E_R^{(L)} \cap F_R^{(L)}$ allows us to write, from \eqref{eq:rewrite-gradients}:
\begin{equation*}
    \overbar{G}_s^{(L)} = \sum_{k=0}^{L-1} g_{k}^{(L)} \one_{t_k \leq s < t_{k+1}} = \sum_{k=0}^{L-1} \left( J_{k}^{(L)} \nabla_x \ftrue(x) + J_{k}^{(L)} \left( g_0^{(L)} - \nabla_x \ftrue(x) \right)  \right ) \one_{t_k \leq s < t_{k+1}}.
\end{equation*}
We first estimate, using the identity $g_0^{(L),\,x} = \nabla_x h_L^{(L),\,x}$,
\begin{align*}
&\E\left[ \sup_{0\leq k' < L} \norm{ \sum_{k=k'}^{L} \left( W^A_{t_{k+1}} - W^A_{t_{k}} \right) J_k^{(L)} \left( g_0^{(L)} - \nabla_x \ftrue(x) \right) }^2 \one_{E^{(L)}_R \cap F_R^{(L)}} \right] \\
&\leq \E\left[ \norm{ \nabla_x \hspace{-2pt} \left( h_L^{(L),\, x} - \ftrue(x) \right) }^4 \right]^{1/2} \E\left[ \sup_{0\leq k' < L}  \norm{ \sum_{k=k'}^L \left( W^A_{t_{k+1}} - W^A_{t_{k}} \right)  J_k^{(L)} }^4 \one_{E^{(L)}_R \cap F_R^{(L)}} \right]^{1/2} \\
&\leq C L^{-2-\zeta/2} \E\left[ \left( \sum_{k=0}^L \norm{ J_k^{(L)} }^2 \right)^2 \one_{E^{(L)}_R \cap F_R^{(L)}} \right]^{1/2} \leq C L^{-\zeta/2}. 
\end{align*}
The second inequality above follows by Burkholder-Davis-Gundy inequality as $J_k^{(L)}$ is adapted, and the last inequality holds by Assumption \ref{ass:backward}. Next, we use Doob's inequality on the main term:
\begin{align*}
&\E\left[ \sup_{0\leq t < 1} \norm{ \int_t^T \left( \sum_{k=0}^{L-1} J_{k}^{(L)} \nabla_x \ftrue(x) \one_{t_k \leq s < t_{k+1}} - G_s \right) \dd W^A_s   }^2  \one_{E^{(L)}_R \cap F_R^{(L)}} \right] \\
&\leq C \, \E\left[ \int_0^T \norm{ \sum_{k=0}^{L-1} J_{k}^{(L)} \nabla_x \ftrue(x) \one_{t_k \leq s < t_{k+1}} - G_s  }^2 \dd s  \,\, \one_{E^{(L)}_R \cap F_R^{(L)}} \right] \\
&\leq C \, \E\left[ \int_0^T \norm{ \overbar{G}_s^{(L)} - G_s  }^2 \dd s  \,\, \one_{E^{(L)}_R} \right] + C \Delta_L  \E \left[ \norm{ \nabla_x \hspace{-2pt} \left( h_L^{(L),\, x} - \ftrue(x) \right) }^2 \sum_{k=0}^{L-1} \norm{J_k^{(L)}}^2  \one_{E^{(L)}_R \cap F_R^{(L)}} \right] \\
&\leq C \, \E\left[ \int_0^T \norm{ \overbar{G}_s^{(L)} - G_s  }^2 \dd s  \,\, \one_{E^{(L)}_R} \right] + C L^{-1-\zeta/2}.
\end{align*}
Combining the two results, we get
\begin{equation} \label{eq:estimaton-ito-EF} 
    \eqref{eq:ito-integral-cond-EF} \leq C \, \E\left[ \int_0^T \norm{ \overbar{G}_s^{(L)} - G_s  }^2 \dd s  \,\, \one_{E^{(L)}_R \cap F^{(L)}_R  } \right] + C L^{-\zeta/2}.  
\end{equation}

\noindent \underline{Step 7: Bound the quadratic covariation error term.} Recall from \eqref{eq:unif-bound-tilde-2} that we need to estimate 
\begin{equation} \label{eq:remainder-covar}
 \E \left[ \sup_{0\leq t < 1} \norm{ \left[W^A, G \right]_{\cdot} \Big\vert^{T}_{t} - \sum_{k>Lt-1} \Delta W^A_k  \Delta \overbar{G}_{k}^{(L)} }^2 \one_{E^{(L)}_R \cap F^{(L)}_R} \right].
\end{equation}
We first transform \eqref{eq:remainder-covar} into a forward problem:
\begin{equation*}
\eqref{eq:remainder-covar} \leq 2 \,  \E \left[ \sup_{0\leq t < 1} \norm{ \left[W^A, G\right]_{t} - \sum_{k\leq Lt-1} \Delta W^A_k  \Delta \overbar{G}_{k}^{(L)} }^2 \one_{E^{(L)}_R \cap F^{(L)}_R} \right].
\end{equation*}
We know that $W^A$ is a continuous martingale, but $G$ is only a continuous semimartingale. To deal with the quadratic covariation term, we decompose $G = G^M + G^{BV}$, where $G^M$ is a continuous martingale and $G^{BV}$ is an adapted process of bounded variation \cite{protter2005stochastic}. We can then write $\left[W^A, G\right] = \left[W^A, G^M\right]$, and 
\begin{align}
\left[W^A, G\right]_{t} - \sum_{k\leq Lt-1} \Delta W^A_k  \Delta \overbar{G}_{k}^{(L)} &= \left[W^A, G^M\right]_{t} - \sum_{k\leq Lt-1} \Delta W^A_k  \Delta G^M_{k} \nonumber \\
&+ \sum_{k\leq Lt-1} \Delta W^A_k \left( \Delta G_k - \Delta \overbar{G}_{k}^{(L)} - \Delta G^{BV}_k \right) \label{eq:discrete-covar}
\end{align}

\noindent \textbf{Claim:} The following process is a martingale:
\begin{align*}
\widetilde{M}_s &\coloneqq\left[W^A, G^M \right]_s - \left(W^A_s - W^A_{t_{k_s}} \right) \left(G^M_s - G^M_{t_{k_s}} \right) - \sum_{k\leq Ls-1} \Delta W^A_{k} \Delta G^M_{k}.
\end{align*}
\textit{Proof of the Claim:} We use the fact that $W^A$, $G^M$, and $\left[ W^A, G^M \right] - W^A G^M$ are all martingales. If $t_k \leq s < t < t_{k+1}$, then
\begin{align*}
\expect{ \widetilde{M}_t - \widetilde{M}_s | \FF_s } &=  \E \left[ \left[W^A, G^M \right]_{t} - W^A_t G^M_t \Big\vert\, \FF_s \right] + W^A_k \E\left[ G^M_t \Big\vert\, \FF_s \right] + \E\left[ W^A_t \Big\vert\, \FF_s \right] G^M_k  \\
&\quad - \left( \left[W^A, G^M \right]_s -  W^A_s G^M_s + W^A_{k} G^M_s + W^A_s G^M_k \right) \\
&= 0.
\end{align*}
Next, we compute, using the tower law,
\begin{align*}
\expect{ \widetilde{M}_{t_{k+1}} - \widetilde{M}_{t_k} | \FF_{t_k} } &=  \E \left[  \left[W^A, G^M \right]_{\cdot} \Big\vert^{t_{k+1}}_{t_k} \Big\vert\, \FF_{t_k} \right] - \expect{ \Delta W^A_{k} \Delta G^M_{k} | \FF_{t_k} } \\
&= \E\left[ W^A_{t_{k+1}} G^M_{t_{k+1}} \Big\vert\, \FF_{t_k} \right] - W^A_{t_k} G^M_{t_k} - \E\left[ \Delta W^A_{k} \Delta G^M_{k} \Big\vert\, \FF_{t_k} \right] = 0.
\end{align*}
Finally, we check that for $t_k \leq s < t_{k+1}$, we also have
\begin{align*}
\expect{ \widetilde{M}_{t_{k+1}} - \widetilde{M}_{s} | \FF_{s} } &=  \E \left[  \left[W^A, G^M \right]_{t_{k+1}} \Big\vert\, \FF_{s} \right] - \left[W^A, G^M \right]_{s} + \left(W^A_s - W^A_{t_k} \right) \left(G^M_s - G^M_{t_{k}} \right) \\
&\quad- \E \left[ W^A_{t_{k+1}} G^M_{t_{k+1}} \Big\vert\, \FF_{s} \right] + W^A_{s} G^M_{t_k} +  W^A_{t_k} G^M_{s} - W^A_{s} G^M_s  \\
&= 0.
\end{align*}
\qedwhite


\noindent We can now rewrite \eqref{eq:discrete-covar} as 
\begin{align}
\left[W^A, G\right]_{t} - \sum_{k\leq Lt-1} \Delta W^A_k  \Delta \overbar{G}_{k}^{(L)} &= \widetilde{M}_t + \underbrace{ \left(W^A_s - W^A_{t_{k_s}} \right) \left(G^M_s - G^M_{t_{k_s}} \right) }_{\tcircle{1}} -  \sum_{k\leq Lt-1} \underbrace{ \Delta W^A_k \Delta G^{BV}_k }_{\tcircle{2}}  \nonumber \\
&+  \sum_{k\leq Lt-1} \underbrace{ \left( \Delta W^A_{k-1} - \Delta W^A_{k} \right) \left( G_k - \overbar{G}_{k}^{(L)} \right) }_{\tcircle{3}}. \label{eq:discrete-covar-2}
\end{align}
First, the following estimations are straightforward:
\begin{align}
\E \left[ \sup_{0\leq t < 1} \norm{ \tcircle{1} }^2 \right] &\leq C \E \left[ \sup_{0\leq t < 1} \norm{G_t}^4 \right]^{1/2} \E \left[ \sup_{0\leq t < 1} \norm{W^A_s - W^A_{t_{k_s}}}^4 \right]^{1/2} \leq C L^{-1/2}, \nonumber \\
\E \left[ \sup_{0\leq t < 1} \norm{ \sum_{k\leq Lt-1} \tcircle{2} \, }^2 \right] &\leq \E \left[ \sup_{0\leq k < L} \norm{\Delta W^A_k}^2 \left( \sum_{k=0}^{L-1} \norm{ \Delta G^{BV}_k } \right)^2 \right] \leq CL^{-1/2}. \label{eq:step7-estimation1-2}
\end{align}
Next, we use Doob's martingale inequality to estimate
\begin{align*}
\E \left[ \sup_{0\leq t < 1} \norm{\widetilde{M}_t}^2 \right] \leq C \E \left[ \norm{\widetilde{M}_T}^2 \right] = C \E\left[ \norm{\left[W^A, G^M \right]_T - \sum_{k=0}^{L-1} \Delta W^A_{k} \Delta G^M_{k}}^2 \right].
\end{align*}
As $W^A$ and $G^M$ are martingales that can be represented as stochastic integrals with respect to Brownian motion, the oscillations of the squared increments of $W^A$ and $G^M$ around their mean are vanishing like $L^{-1/2}$, see \cite[Theorem 1]{wong1965}. That means:
\begin{equation} \label{eq:step7-estimation-M}
    \E \left[ \sup_{0\leq t < 1} \norm{\widetilde{M}_t}^2 \right] \leq C L^{-1/2}.
\end{equation}
Finally, we use similar arguments to Step 6 to derive an upper bound for the last term
\begin{equation*}
\E \left[ \sup_{0\leq t < 1} \norm{ \sum_{k \leq Lt-1} \tcircle{3} \, }^2 \one_{E^{(L)}_R \cap F^{(L)}_R} \right] \leq C \E\left[ \int_0^T \norm{ \overbar{G}_s^{(L)} - G_s  }^2 \dd s  \,\, \one_{E^{(L)}_R \cap F^{(L)}_R  } \right] + C L^{-\zeta/2}.
\end{equation*}
We plug this last inequality together with \eqref{eq:step7-estimation1-2} and \eqref{eq:step7-estimation-M} back into \eqref{eq:remainder-covar} and \eqref{eq:discrete-covar-2} to get 
\begin{equation} \label{eq:upper-bound-covar}
\eqref{eq:remainder-covar} \leq C \, \E\left[ \int_0^T \norm{ \overbar{G}_s^{(L)} - G_s  }^2 \dd s \right] + C L^{-\min(1, \zeta)/2}.
\end{equation}


\noindent \underline{Step 8: Prove that the remainder $R^{(L)}_k$ uniformly vanishes.} We proceed to show that
\begin{equation} \label{eq:remainder-taylor}
    \E\left[ \sup_{0\leq t\leq 1} \norm{ \sum_{k > Lt-1} R_k^{(L)} \hspace{-2pt} \left( g_{k+1}^{(L)} \right) }^2  \one_{E^{(L)}_R \cap F^{(L)}_R} \right] \leq C(1+R^4) L^{-1},
\end{equation}
which is straightforward since:
\begin{align*}
    &\E\left[ \sup_{0\leq t\leq 1} \norm{ \sum_{k > Lt-1} R_k^{(L)} \hspace{-2pt} \left( g_{k+1}^{(L)} \right) }^2  \one_{E^{(L)}_R \cap F^{(L)}_R} \right] \leq \E\left[ \left( \sum_{k=0}^{L-1} \norm{R_k^{(L)} \hspace{-2pt}\left( g_{k+1}^{(L)} \right) } \right)^2 \one_{E^{(L)}_R} \right] \\
    &\leq C \E\left[ \left( \sum_{k=0}^{L-1} \left( \norm{A_k^{(L)}} R + \norm{b_k^{(L)}} \right)^2  \norm{A_k^{(L)}} \norm{ g_{k+1}^{(L)} } \right)^2 \right] \\
    &\leq C L \, \E\left[ \sup_k \norm{g_k^{(L)}}^2 \sum_{k=0}^{L-1} \left( \norm{A_k^{(L)}} R + \norm{b_k^{(L)}} \right)^4 \norm{A_k^{(L)}}^2 \right] \\
    &\leq C L^2 \E\left[ \sup_k \norm{g_k^{(L)}}^4 \right]^{1/2} \E\left[ \sum_{k=0}^{L-1} \left( \norm{A_k^{(L)}} R + \norm{b_k^{(L)}} \right)^8 \norm{A_k^{(L)}}^4 \right]^{1/2} \leq C(1+R^4) L^{-1}.
\end{align*}


\noindent \underline{Step 9: Prove that the remainder $N^{(L),1}_k$ uniformly vanishes.} First note that we can write $N^{(L), 1}_{k, ij} \hspace{-2pt} \left( g \right) = \sum_{l,m=1}^d N^{(L), 1}_{k, ij, lm} \hspace{-2pt} \left( g \right)$, where 
\begin{align} \label{eq:N-kijl}
    N^{(L), 1}_{k, ij, lm} \hspace{-2pt} \left( g \right) &\coloneqq \left( A^{(L)}_{k, im} A^{(L)}_{k, il} h^{(L)}_{k, m} - \left(\Sigma^A_{t_k}\right)_{imil} H_{t_k, m} L^{-1} \right) g_{lj}.
\end{align}
Thus, we get
\begin{align*}
\E \left[ \sup_{0\leq t \leq T}  \abs{ \sum_{k > Lt-1} N_{k, ij}^{(L), 1} \hspace{-2pt} \left( g_{k+1}^{(L)} \right) }^2\one_{E^{(L)}_R \cap F^{(L)}_R} \right] &\leq d^2 \sum_{l,m=1}^d \E\left[ \sup_{0\leq t \leq T}  \abs{ \sum_{k > Lt-1} N_{k, ij, lm}^{(L), 1} \hspace{-2pt} \left( g_{k+1}^{(L)} \right) }^2 \one_{E^{(L)}_R \cap F^{(L)}_R}  \right]. \\
\end{align*}
We now expand \eqref{eq:N-kijl} using the definition of Hypothesis \ref{hypothesis.2}.
\begin{align*}
    N^{(L), 1}_{k, ij, lm}\left( g \right) &= \underbrace{ \left( \left( \Delta W^A_k \right)_{im} \left( \Delta W^A_k \right)_{il} - \int_{t_k}^{t_{k+1}} \expect*{ \left(\Sigma^A_s\right)_{imil} | \GG_{k-1}}  \dd s \right) h^{(L)}_{k,m} \, g_{lj} }_{\tcircle{1}}  \\
    &+ \underbrace{ h^{(L)}_{k,m} \int_{t_k}^{t_{k+1}} \expect*{ \left(\Sigma^A_s - \Sigma^A_{t_k} \right)_{imil} | \GG_{k-1}}  \dd s }_{\tcircle{2}} + \underbrace{ \left(\Sigma^A_{t_k}\right)_{imil} \left( h^{(L)}_{k,m} - H_{t_k, m} \right) L^{-1} }_{\tcircle{3}} \\
    &+ \underbrace{ \left[ \left( \overbar{A}_{t_k}\right)_{im} \left( \Delta W^A_k \right)_{il} + \left( \overbar{A}_{t_k}\right)_{il} \left( \Delta W^A_k \right)_{im}  \right] h^{(L)}_{k,m} L^{-1} }_{\tcircle{4}} + \underbrace{ \left( \overbar{A}_{t_k}\right)_{im} \left( \overbar{A}_{t_k}\right)_{il} h^{(L)}_{k,m} L^{-2} }_{\tcircle{5}} 
\end{align*}
We show the estimate on $\tcircle{1}$ in Steps 11 and the estimates on $\tcircle{2}$--$\tcircle{5}$ in Step 12. \\

\noindent \underline{Step 10: Preliminary lemmas to estimate the term $\tcircle{1}$.} We first bound the moments of a product of two correlated Gaussian random variables. 

\begin{lem} \label{lemma:moment-gaussian}
Let $\sigma>0$ and $Z_1, Z_2 \sim N(0, \sigma^2)$. Then for any real number $r>1$, \[
    \E\left[ \left( Z_1 Z_2 - \E\left[ Z_1 Z_2 \right] \right)^r \right] \leq C_r \, \sigma^{2r},  
\]
where $C_r$ is a constant depending only on $r$.
\end{lem}
\begin{proof}
Define $Y_1 \coloneqq \frac{1}{2}(Z_1 + Z_2)$ and $Y_2 \coloneqq \frac{1}{2}(Z_1 - Z_2)$. We have, for $i=1,2$, $Y_i \sim \NN(0, \sigma_i^2)$, where $\sigma_i \leq \sigma$. But $Z_1Z_2 = Y_1^2 - Y_2^2$, so
\begin{align*}
    \E\left[ \left( Z_1 Z_2 - \E\left[ Z_1 Z_2 \right] \right)^r \right] &= \E\left[ \left( \left( Y_1^2 - \E\left[Y_1^2\right] \right) - \left( Y_2^2 - \E\left[Y_2^2\right] \right) \right)^r \right] \\
    &\leq 2^{r-1} \E\left[ \left( Y_1^2 - \E\left[Y_1^2\right] \right)^r + \left( Y_2^2 - \E\left[Y_2^2\right] \right)^r \right] \\
    &\leq 2^{r-1} \E\left[ Y_1^{2r} + Y_2^{2r} \right] \\
    &= \frac{C_r}{2} \left( \sigma_1^{2r} + \sigma_2^{2r}  \right) \leq C_r \sigma^{2r}
\end{align*}
We use Minkowski inequality, the fact that $x\mapsto x^n$ is increasing on the positive reals, and the formula for moments of centered Gaussian random variable.  

\end{proof}

\noindent We will apply in the next step a version of the discrete Gronwall lemma. The proof is straightforward and omitted for clarity.

\begin{lem} \label{lemma:gronwall}
    Let $u > 0$ and $(v_n)_{n\in \N} \subset \R_{>0}$. Then, if $e_{n+1} \leq u e_n + v_n$ for each $n\geq 0$, we have 
    \[
        e_n \leq u^n e_0 + \sum_{n'=0}^{n-1} u^{n-1-n'} v_{n'}.
    \]
\end{lem}

\noindent \underline{Step 11: Prove that the term $\tcircle{1}$ uniformly vanishes.}  We can now finish the argument with a similar martingale argument as in the proof of Theorem~\ref{thm:H2}. Define now, for $k=0, \ldots, L-1$, (we omit the indices for clarity) 
\begin{equation*}
    X_k^{(L)} \coloneqq 
    \begin{cases}
    \left( \left( \Delta W^A_k \right)_{im} \left( \Delta W^A_k \right)_{il} - \int_{t_k}^{t_{k+1}} \expect*{ \left(\Sigma^A_s\right)_{imil} | \GG_{k-1}}  \dd s \right) h^{(L)}_{k,m} \, J^{(L)}_{k, ln} \quad &\mbox{on} \,\, E^{(L)}_{k, R} \cap F^{(L)}_{k-1, R} \\
    0 &\mbox{elsewhere}.
    \end{cases}
\end{equation*}
Then, as $E^{(L)}_R \cap F^{(L)}_R \subseteq E^{(L)}_{k, R} \cap F^{(L)}_{k-1, R}$,
\begin{align}
\E\left[ \sup_{0\leq t\leq T} \abs{ \sum_{k>Lt-1} \tcircle{1} \, }^2 \one_{E^{(L)}_R \cap F^{(L)}_R} \right] &=\E\left[ \sup_{0\leq t \leq T}  \abs{ \sum_{k > Lt-1} X_k^{(L)} g^{(L)}_{0, nj} }^2 \one_{E^{(L)}_R \cap F^{(L)}_R}  \right] \nonumber \\
&\leq \E\left[ \norm{ g_0^{(L)} }^2 \sup_{0\leq t \leq T}  \abs{ \sum_{k > Lt-1} X_k^{(L)} }^2 \one_{E^{(L)}_R \cap F^{(L)}_R}  \right] \nonumber \\
&\leq \E\left[ \norm{ g_0^{(L)} }^4 \right]^{1/2} \E\left[ \sup_{0\leq t \leq T}  \abs{ \sum_{k > Lt-1} X_k^{(L)} }^4 \one_{E^{(L)}_R \cap F^{(L)}_R}  \right]^{1/2}. \label{eq:remainder-1}
\end{align}
Now, by Minkowski inequality, we get
\begin{align}
    \E\left[ \sup_{0\leq t \leq T}  \abs{ \sum_{k > Lt-1} X_k^{(L)} }^4 \one_{E^{(L)}_R \cap F^{(L)}_R}  \right] &\leq 8 \, \E\left[ \left( \abs{ \sum_{k=0}^{L-1} X_k^{(L)} }^4 +  \sup_{0\leq t \leq T} \abs{ \sum_{k \leq Lt-1} X_k^{(L)} }^4 \right) \one_{E^{(L)}_R \cap F^{(L)}_R}  \right] \nonumber \\
    &\leq 16 \, \E\left[ \sup_{0\leq k < L}  \abs{ \sum_{k' \leq k} X_{k'}^{(L)} }^4 \right] \label{eq:remainder-2}
\end{align}
Define now $S_k^{(L)} \coloneqq \sum_{k'=0}^k X_{k'}^{(L)}$. As $X_k^{(L)}$ is $\GG_k-$measurable, with $\expect*{ X_k^{(L)} | \GG_{k-1} } = 0$, we deduce that $S_k^{(L)}$ is a $\GG_{k}-$martingale so by Doob's martingale inequality, 
\begin{equation} \label{eq:doobs-sk}
\E\left[ \sup_{k} \abs{ S_k^{(L)} }^4 \right] \leq \left(\frac{4}{3}\right)^4 \E\left[ \abs{ S_L^{(L)} }^4\right].
\end{equation}
To further estimate the latter, observe that 
\begin{align*}
    \expect*{ \left( S_{k}^{(L)} \right)^4 | \GG_{k-1} } &= \left( S_{k-1}^{(L)} \right)^4 + 4 S_{k-1}^3 \expect*{ X_{k}^{(L)} | \GG_{k-1}} + 6 S_{k-1}^2 \expect*{ \left( X_{k}^{(L)} \right)^2 | \GG_{k-1}} \\
    &+ 4 S_{k-1} \expect*{ \left( X_{k}^{(L)} \right)^3 | \GG_{k-1}} + \expect*{ \left( X_{k}^{(L)} \right)^4 | \GG_{k-1}}.
\end{align*}
Using the fact that $h_k^{(L)}, J_k^{(L)}$, and $E^{(L)}_{k, R} \cap F^{(L)}_{k-1, R}$ are $\GG_{k-1}-$measurable and that $\Delta W^k_A \mid \GG_{k-1}$ is normally distributed with variance $\OO(L^{-1})$ almost surely, we can use Lemma~\ref{lemma:moment-gaussian} and take expectations to deduce that
\begin{align*}
    \E\left[ \left( S_{k}^{(L)} \right)^4 \right] &\leq \E\left[ \left( S_{k-1}^{(L)} \right)^4 \right] + C L^{-2} \E \left[ S_{k-1}^2 \left( h_{k,m}^{(L)} J_{k, ln}^{(L)} \right)^2 \one_{E^{(L)}_{k, R} \cap F^{(L)}_{k-1, R}}\right] \\
    &+ C L^{-3} \E \left[ S_{k-1} \left( h_{k,m}^{(L)} J_{k, ln}^{(L)} \right)^3 \one_{E^{(L)}_{k, R} \cap F^{(L)}_{k-1, R}} \right] + C L^{-4} \E \left[ \left( h_{k,m}^{(L)} J_{k, ln}^{(L)} \right)^4 \one_{E^{(L)}_{k, R} \cap F^{(L)}_{k-1, R}} \right].
\end{align*}
We use Young's inequalities $\delta^2 ab = \delta^{1/2}a \cdot \delta^{3/2}b \leq \frac{1}{2} \delta a^2 + \frac{1}{2} \delta^3 b^2$ and $\delta^3 ab = \delta^{1/4}a \cdot \delta^{11/4}b \leq \frac{1}{4} \delta a^4 + \frac{3}{4} \delta^{11/3} b^{4/3}$ to obtain
\begin{equation*}
    \E\left[ \left( S_{k}^{(L)} \right)^4 \right] \leq \left(1 + C L^{-1} \right) \E\left[ \left( S_{k-1}^{(L)} \right)^4 \right] + C L^{-3} \E \left[ \left( h_{k,m}^{(L)} J_{k, ln}^{(L)} \right)^4 \one_{E^{(L)}_{k, R} \cap F^{(L)}_{k-1, R}} \right].
\end{equation*}
Hence, by Lemma~\ref{lemma:gronwall} and $S_{-1} = 0$, we conclude that
\begin{equation*}
\E\left[\abs{ S_{k}^{(L)} }^4 \right] \leq C L^{-3} \sum_{k'=0}^{k} \E \left[ \left( h_{k',m}^{(L)} J_{k', ln}^{(L)} \right)^4 \one_{E^{(L)}_{k', R} \cap F^{(L)}_{k'-1, R}} \right].
\end{equation*}
Observe now that since $J_k^{(L)} = \left( \del h_k^{(L)} / \, \del x \right)^{-1}$,
\begin{equation*}
\E \left[ \left( J_{k, ln}^{(L)} \right)^4 \one_{E^{(L)}_{k, R} \cap F^{(L)}_{k-1, R}} \right] \leq \E \left[ \norm{ \left( \del h_k^{(L)} / \, \del x \right)^{-1} }^4 \one_{E^{(L)}_{k, R} \cap F^{(L)}_{k-1, R}} \right].
\end{equation*}
\iffalse
{\color{red}{\bf Alternative:} When $R \ge 2\,C_1$ with $C_1 = \left( 1 + 2\abs{\sigma''(0)} + 2 \sup \abs{\sigma'''} \right)$,
\begin{eqnarray}
&&\E \left[ \norm{ J_{k}^{(L)} }^4 \one_{E^{(L)}_{k, R} \cap F^{(L)}_{k-1, R}} \right] = \E \left[ \norm{ \prod_{k'=0}^{k-1} \left( I_d + D_{k'}^{(L)} \right)^{-1}  }^4 \one_{E^{(L)}_{k, R} \cap F^{(L)}_{k-1, R}} \right]\\
&\leq& \prod_{k'=0}^{k-1} \E \left[ \norm{ \left( I_d + D_{k'}^{(L)} \right)^{-1}  }^4 \one_{\tilde{E}^{(L)}_{k, R} \cap \tilde{F}^{(L)}_{k-1, R}} \right] \leq \left(1+\frac{C_1}{R-C_1}\right)^k.
\end{eqnarray}
The last inequality holds due to Lemma 4-(iii).
}
\fi
Hence, we deduce from \eqref{eq:remainder-1}, \eqref{eq:remainder-2}, \eqref{eq:doobs-sk} and Assumption~\ref{ass:backward} that 
\begin{equation} \label{eq:bound-circle-1} 
    \E\left[ \sup_{0\leq t\leq T} \abs{ \sum_{k>Lt-1} \tcircle{1} \, }^2 \one_{E^{(L)}_R \cap F^{(L)}_R} \right] \leq C R^2 L^{-1}.
\end{equation}

\noindent \underline{Step 12: Prove that the terms $\tcircle{2}, \tcircle{3}, \tcircle{4}$ and $\tcircle{5}$ uniformly vanish.} A direct estimation gives
\begin{align}
    \E\left[ \sup_{0\leq t\leq T} \abs{ \sum_{k>Lt-1} \tcircle{2} \, }^2 \one_{E^{(L)}_R} \right] &\leq \E\left[ \left( \sum_{k=0}^{L-1} \abs{\tcircle{2}} \right)^2 \one_{E^{(L)}_R} \right] \nonumber \\
    &\leq \E\left[ R^2 \left( \sum_{k=0}^{L-1} \int_{t_k}^{t_{k+1}} \expect*{ \abs{ \Sigma^A_s - \Sigma^A_{t_k} }_{imil} | \GG_{k-1}}  \dd s \right)^2 \right] \nonumber \\
    &\leq  R^2\left( \int_{0}^{T}  \abs{t_{k_s} - s}^{\kappa/2} \dd s \right)^2 \leq C R^2 L^{-\kappa}. \label{eq:bound-circle-2}
\end{align}

\noindent Next, we use the proof of Theorem~\ref{thm:H2} establishing that the rate of uniform $L^2$ convergence of $h_{\floor{Lt}}^{(L)}$ to $H_t$ as $L\to\infty$ is $L^{-\min(1, \kappa)}$.
\begin{align}
    \E\left[ \sup_{0\leq t\leq T} \abs{ \sum_{k>Lt-1} \tcircle{3} \, }^2 \one_{E^{(L)}_R} \right] &\leq L^{-2} \E\left[ \left( \sum_{k=0}^{L-1} \abs{ \Sigma^A_{t_k, imil}} \abs{h_{k,m}^{(L)} - H_{t_k, m}} \right)^2 \right] \nonumber \\
    &\leq C L^{-2} \E\left[ L^2 \sup_{k} \norm{ h_k^{(L)} - H_{t_k}}^2 \right] \leq C L^{-\min(1, \kappa)}. \label{eq:bound-circle-3}
\end{align}

\noindent Again, a direct computation and Cauchy-Schwarz gives
\begin{align}
    \E\left[ \sup_{0\leq t\leq T} \abs{ \sum_{k>Lt-1} \tcircle{4} \, }^2 \one_{E^{(L)}_R} \right] &\leq R^2L^{-2} \E\left[ \left( \sum_{k=0}^{L-1} \Big| \left( \overbar{A}_{t_k}\right)_{im} \left( \Delta W^A_k \right)_{il} + \left( \overbar{A}_{t_k}\right)_{il} \left( \Delta W^A_k \right)_{im} \Big| \right)^2 \right] \nonumber \\
    &\leq C R^2 L^{-1} \E\left[ \sum_{k=0}^{L-1} \left( \Delta W^A_k \right)^2_{il} + \left( \Delta W^A_k \right)^2_{im}  \right] \nonumber \\
    &\leq C R^2 L^{-1}. \label{eq:bound-circle-4}
\end{align}

\noindent Finally, the last term is straightforward to bound:
\begin{equation}
\E\left[ \sup_{0\leq t\leq T} \abs{ \sum_{k>Lt-1} \tcircle{5} \, }^2 \one_{E^{(L)}_R} \right] \leq R^2 L^{-4} \E\left[ \left( \sum_{k=0}^{L-1} \abs{ \left( \overbar{A}_{t_k}\right)_{im} \left( \overbar{A}_{t_k}\right)_{il} } \right)^2 \right] \leq C R^2 L^{-2}. \label{eq:bound-circle-5}
\end{equation}

\noindent \underline{Step 13: Prove that the remainder $N^{(L),2}_k$ uniformly vanishes.} We proceed to show that
\begin{equation} \label{eq:remainder-N2}
    \E\left[ \sup_{0\leq s < 1} \norm{ \sum_{k > Ls-1} N^{(L),2}_{k} \hspace{-2pt} \left(g_{k+1}^{(L)} \right) }^2  \one_{E^{(L)}_R \cap F^{(L)}_R} \right] \leq C R^2 L^{-\min(1,\kappa)}.
\end{equation}
The computations are similar to $N^{(L),1}_k$, although less involved. {\color{blue}Hence we omit the proof for \eqref{eq:remainder-N2}.} \\ %For the sake of the length of the proof, we leave this part to the reader. \\

\noindent \underline{Step 14: Prove that the remainder $N^{(L),3}_k$ uniformly vanishes.} We proceed to show that
\begin{equation} \label{eq:remainder-N3}
    \E\left[ \sup_{0\leq s < 1} \norm{ \sum_{k > Ls-1} N^{(L),3}_{k} \hspace{-2pt} \left(g_{k+1}^{(L)} \right) }^2  \one_{E^{(L)}_R \cap F^{(L)}_R} \right] \leq C L^{-\min(1,\kappa)}.
\end{equation}
First, we note that from \eqref{eq:D_R_N}
\begin{equation*}
\sum_{k > Ls-1} N^{(L),3}_{k} \hspace{-2pt} \left(g_{k+1}^{(L)} \right) =  \sum_{k > Ls-1} \left( \overbar{A}_{t_k} + \frac{1}{2} \sigma''(0) \frac{\del Q}{\del x}(t_k, H_{t_k} ) \right) \left( g_{k+1}^{(L)} - g_{k}^{(L)} \right) L^{-1}.
\end{equation*}
We can rewrite the first term using a telescoping sum:
\begin{align*}
\sum_{k > Ls-1} \overbar{A}_{t_k} \left( g_{k+1}^{(L)} - g_{k}^{(L)} \right) = \left( \overbar{A}_{T} g_{L}^{(L)} - \overbar{A}_{t_{k_s}} g_{t_{k_s+1}}^{(L)} \right) + \sum_{k>Ls-1} \left( \overbar{A}_{t_{k}} - \overbar{A}_{t_{k+1}} \right) g_{k+1}^{(L)}.
\end{align*}
Hence, we deduce the following bound using Assumptions \eqref{ass:ito} and \eqref{ass:backward}
\begin{align*}
    &\E\left[ \sup_{0\leq s < 1} \norm{ \sum_{k > Ls-1} \overbar{A}_{t_k} \left( g_{k+1}^{(L)} - g_{k}^{(L)} \right) }^2  \right] \\
    &\leq C \, \E\left[ \sup_{0 \leq k < L} \norm{g_k^{(L)}}^2 \right] + CL \E\left[ \sup_{0\leq k < L} \norm{g_k^{(L)}}^2 \sum_{k=0}^{L-1} \norm{\overbar{A}_{t_{k}} - \overbar{A}_{t_{k+1}}}^2  \right] \leq C (1+ L^{2-\kappa}).
\end{align*}
Similar computations are performed on the second term, using the fact that $(H_t)_{t\in\left[0,1\right]}$ has a.s $\gamma-$H\"older-continuous paths, for all $\gamma<\kappa+1/2$ (see the proof of Lemma~\ref{lem:drift-lipschitz}). \\
%using the fact that the quadratic variation of $H$ is finite. \\


\noindent \underline{Step 15: Fix $R$ and $\delta$, and finish the proof.} From equation \eqref{eq:remainder-taylor}, \eqref{eq:bound-circle-1}, \eqref{eq:bound-circle-2}, \eqref{eq:bound-circle-3}, \eqref{eq:bound-circle-4}, \eqref{eq:bound-circle-5}, \eqref{eq:remainder-N2}, \eqref{eq:remainder-N3}, and $R>1$, we deduce that  
\begin{equation} 
\E\left[ \sup_{0\leq t\leq 1} \norm{ \sum_{k > Lt-1} D_k^{(L)} \hspace{-2pt} \left( g_{k+1}^{(L)} \right) }^2  \one_{E^{(L)}_R \cap F^{(L)}_R }  \right] \leq C R^4 L^{-\min(1, \kappa)}. \label{eq:bound-remainder-total}
\end{equation}
We plug \eqref{eq:estimaton-ito-EF}, \eqref{eq:upper-bound-covar}, and \eqref{eq:bound-remainder-total} into \eqref{eq:unif-bound-tilde-2}, together with Tonelli's theorem, to get
\begin{align*}
    &\mathbb{E}\left[ \sup_{0 \leq t \leq 1} \norm{G_t - \widetilde{G}^{(L)}_t}^2 \one_{E^{(L)}_R \cap F^{(L)}_R } \right] \\
    &\leq C_1 \, \E\left[ \int_0^T \norm{\overbar{G}_s^{(L)} - G_s}^2 \dd s \,\,  \one_{E^{(L)}_R \cap F^{(L)}_R } \right] + C R^4 L^{-\min(1/2,\,\kappa,\, \zeta/2)} \\
    &\leq C_1 \, \E\left[ \int_0^T \norm{G_s - \widetilde{G}_s^{(L)}}^2 \dd s \,\,  \one_{E^{(L)}_R \cap F^{(L)}_R } \right] + C_2 R^4 L^{-\min(1/2,\,\kappa,\, \zeta/2)}. 
\end{align*}
We use \eqref{eq:unif-bound-bar-tilde} for the last inequality. We then apply Gronwall's inequality to deduce that 
\begin{equation*} 
\E\left[ \sup_{0\leq t \leq 1} \norm{G_t - \widetilde{G}^{(L)}_t}^2  \one_{E^{(L)}_R \cap F^{(L)}_R} \right] \leq C_2 R^4 L^{-\min(1/2,\, \kappa,\, \zeta/2)} e^{C_1}.
\end{equation*}
Finally, we plug the last inequality in \eqref{eq:bound-eg} to get
\begin{align*} 
\E\left[ \sup_{0\leq t \leq 1} \norm{G_t - \widetilde{G}^{(L)}_t}^2 \right] &\leq C_3 R^4 L^{-\min(1/2,\,\kappa,\, \zeta/2)} + C_4 \delta \\
&\quad +  C_5 \delta^{-2/(p-2)} \left( R^{-p} + L \exp\left( -C_6(LR^{-1} - 1)^2\right) \right).
\end{align*}
We choose $\delta < C_4^{-1} \epsilon$, $R^p > \max(1, \, C_5 \delta^{-2/(p-2)} \epsilon^{-1})$ and $L$ big enough so that the remaining two terms are both less that $\epsilon$. Thus, 
\begin{equation} \label{eq:gronwall-gtilde}
    \E\left[ \sup_{0\leq t \leq 1} \norm{G_t - \widetilde{G}^{(L)}_t}^2 \right] \leq 4 \epsilon.
\end{equation}
Combining \eqref{eq:unif-bound-bar-tilde} and \eqref{eq:gronwall-gtilde} finishes the proof. \qed \\
